LP-Duality Theory and the Cores of Games

LP-duality theory has played a central role in the study of the core, right from its early days to the present time. However, despite the extensive nature of this work, basic gaps still remain. We address these gaps using the following building blocks from LP-duality theory: 1. Total unimodularity (TUM). 2. Complementary slackness conditions and strict complementarity. Our exploration of TUM leads to defining new games, characterizing their cores and giving novel ways of using core imputations to enforce constraints that arise naturally in applications of these games. The latter include: 1. Efficient algorithms for finding min-max fair, max-min fair and equitable core imputations. 2. Encouraging diversity and avoiding over-representation in a generalization of the assignment game. Complementarity enables us to prove new properties of core imputations of the assignment game and its generalizations.

==> talk.tex <==
\section{Talk}
\label{sec.talk}


New Insights into a Half-Century-Old Work: the Core of the Matching Game


\bigskip

The classic 1971 paper of Shapley and Shubik characterized the core of the assignment game using ideas from matching theory and LP-duality theory and their highly non-trivial interplay. 

The core is a quintessential solution concept in cooperative game theory --- it contains all ways of distributing the total worth of a game among agents in such a way that no sub-coalition has incentive to secede from the grand coalition. Additionally, the pristine structural properties of the assignment game make it a paradigmatic setting for studying the intricacies of this solution concept, with a view to tackling profit-sharing in real-life situations. 

We build on the Shapley-Shubik work in two ways: 

1). We study core imputations of the assignment game through the lens of complementarity, thereby obtaining a relationship between the competitiveness of individuals and teams of agents and the amount of profit they accrue. 

2). Whereas the core of the assignment game is always non-empty, that of the general graph matching game can be empty. We show how to salvage the situation via the notion of approximate core.

 
This talk is completely self-contained. It is based on:

https://www.sciencedirect.com/science/article/pii/S0899825622000239?via%3Dihub

https://arxiv.org/pdf/2202.00619.pdf




\newpage


LP-Duality Theory and the Cores of Games


The core is a quintessential solution concept in cooperative game theory and LP-duality theory has played a central role in its study, right from its early days to the present time. The classic 1971 paper of Shapley and Shubik showed the ``right'' way of exploiting this theory --- in the context of characterizing the core of the assignment game. 

The LP-relaxation of this game  has the following key property: the polytope defined by its constraints has integral vertices; in this case, they are matchings in the underlying graph. Similar characterizations for several basic combinatorial optimization games followed; throughout, this property was established by showing that the underlying linear system is totally unimodular (TUM). 

We will first exploit TUM further via a very general formulation due to Hoffman and Kruskal (1956). The way take this methodology to its logical next step is to use total dual integrality (TDI). In the process, we address new classes of games which have their origins in two major theories within combinatorial optimization, namely perfect graphs and polymatroids.

Whereas the core of the assignment game is always non-empty, that of the general graph matching game can be empty. We show how to salvage the situation --- again using LP-duality in a fundamental way. 








